Fastrack: Fast IO for Secure ML using GPU TEEs

As cloud-based ML expands, ensuring data security during training and inference is critical. GPU-based Trusted Execution Environments (TEEs) offer secure, high-performance solutions, with CPU TEEs managing data movement and GPU TEEs handling authentication and computation. However, CPU-to-GPU communication overheads significantly hinder performance, as data must be encrypted, authenticated, decrypted, and verified, increasing costs by 12.69 to 33.53 times. This results in GPU TEE inference becoming 54.12% to 903.9% slower and training 10% to 455% slower than non-TEE systems, undermining GPU TEE advantages in latency-sensitive applications. This paper analyzes Nvidia H100 TEE protocols and identifies three key overheads: 1) redundant CPU re-encryption, 2) limited authentication parallelism, and 3) unnecessary operation serialization. We propose Fastrack, optimizing with 1) direct GPU TEE communication, 2) parallelized authentication, and 3) overlapping decryption with PCI-e transmission. These optimizations cut communication costs and reduce inference/training runtime by up to 84.6%, with minimal overhead compared to non-TEE systems.

==> 3.motivation.tex <==
\todo{this is to justify the AES-GCM 128 in the baseline to decrypt, and data is already in the spreadsheet.} Without GPU TEEs, when remote users transmit data to cloud servers, they can use faster encryption and authentication schemes like AES-GCM-128. With GPU TEEs, remote users have to use stronger schemes, such as AES-GCM-256, which GPU TEE systems use to guarantee the confidentiality and integrity of data outside the TEEs.
